Discrete FEM-BEM coupling with the Generalized Optimized Schwarz Method

The present contribution aims at developing a non-overlapping Domain Decomposition (DD) approach to the solution of acoustic wave propagation boundary value problems based on the Helmholtz equation, on both bounded and unbounded domains. This DD solver, called Generalized Optimized Schwarz Method (GOSM), is a substructuring method, that is, the unknowns of an iteration are associated with the subdomains interfaces. We extend the analysis presented in a previous paper of one of the author to a fully discrete setting. We do not consider only a specific set of boundary conditions, but a whole class including, e.g., Dirichlet, Neumann, and Robin conditions. Our analysis will also cover interface conditions corresponding to a Finite Element Method - Boundary Element Method (FEM-BEM) coupling. In particular, we shall focus on three classical FEM-BEM couplings, namely the Costabel, Johnson-N\'ed\'elec and Bielak-MacCamy couplings. As a remarkable outcome, the present contribution yields well-posed substructured formulations of these classical FEM-BEM couplings for wavenumbers different from classical spurious resonances. We also establish an explicit relation between the dimensions of the kernels of the initial variational formulation, the local problems and the substructured formulation. That relation especially holds for any wavenumber for the substructured formulation of Costabel FEM-BEM coupling, which allows us to prove that the latter formulation is well-posed even at spurious resonances. Besides, we introduce a systematically geometrically convergent iterative method for the Costabel FEM-BEM coupling, with estimates on the convergence speed.

==> macro.tex <==
\makeatletter
\newcommand\RedeclareMathOperator{%
  \@ifstar{\def\rmo@s{m}\rmo@redeclare}{\def\rmo@s{o}\rmo@redeclare}%
}
% this is taken from \renew@command
\newcommand\rmo@redeclare[2]{%
  \begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
  \expandafter\@ifundefined\@gtempa
     {\@latex@error{\noexpand#1undefined}\@ehc}%
     \relax
  \expandafter\rmo@declmathop\rmo@s{#1}{#2}}
% This is just \@declmathop without \@ifdefinable
\newcommand\rmo@declmathop[3]{%
  \DeclareRobustCommand{#2}{\qopname\newmcodes@#1{#3}}%
}
\@onlypreamble\RedeclareMathOperator
\makeatother


\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\mrm}{\mathrm}
\newcommand{\mA}{\mathrm{A}}
\newcommand{\mB}{\mathrm{B}}
\newcommand{\mL}{\mathrm{L}}
\newcommand{\mH}{\mathrm{H}}
\newcommand{\mJ}{\mathrm{J}}
\newcommand{\mV}{\mathrm{V}}
\newcommand{\mW}{\mathrm{W}}
\newcommand{\mM}{\mathrm{M}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\mD}{\mathrm{D}}
\newcommand{\mT}{\mathrm{T}}
\newcommand{\mS}{\mathrm{S}}
\newcommand{\mP}{\mathrm{P}}
\newcommand{\mR}{\mathrm{R}}
\newcommand{\mQ}{\mathrm{Q}}
\newcommand{\mX}{\mathrm{X}}
\newcommand{\mY}{\mathrm{Y}}
\newcommand{\mZ}{\mathrm{Z}}
\newcommand{\mbH}{\mathbb{H}}
\newcommand{\mbV}{\mathbb{V}}
\newcommand{\mbX}{\mathbb{X}}
\newcommand{\Vh}{\mathrm{V}_{h}}
\newcommand{\Wh}{\mathrm{W}_{h}}
\newcommand{\Qh}{\mathrm{Q}_{h}}
\newcommand{\VhO}{\mathrm{V}_{h,0}}
\newcommand{\mbVh}{\mathbb{V}_{h}}
\newcommand{\mbXh}{\mathbb{X}_{h}}
\newcommand{\infsup}{\mathop{\mrm{infsup}}}
\newcommand{\rref}{\textsc{r}}
\newcommand{\bell}{\boldsymbol{\ell}}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}

\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\bl}{\boldsymbol{l}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfff}{\mathbf{f}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\dir}{\textsc{d}}
\newcommand{\neu}{\textsc{n}}
\newcommand{\llangle}{\langle\!\langle}
\newcommand{\rrangle}{\rangle\!\rangle}
\newcommand{\lbr}{\lbrack}
\newcommand{\rbr}{\rbrack}

\newcommand{\ctru}{\mathfrak{u}}
\newcommand{\ctrv}{\mathfrak{v}}
\newcommand{\ctrw}{\mathfrak{w}}
\newcommand{\ctrp}{\mathfrak{p}}
\newcommand{\ctrq}{\mathfrak{q}}
\newcommand{\ctrf}{\mathfrak{f}}
\newcommand{\ctrg}{\mathfrak{g}}
\newcommand{\diff}{\mathop{}\!\mathrm{d}}   % integral measure

%% \newcommand{\ctru}{\boldsymbol{u}}
%% \newcommand{\ctrv}{\boldsymbol{v}}
%% \newcommand{\ctrw}{\boldsymbol{w}}
%% \newcommand{\ctrp}{\boldsymbol{p}}
%% \newcommand{\ctrq}{\boldsymbol{q}}
%% \newcommand{\ctrf}{\boldsymbol{f}}
%% \newcommand{\ctrg}{\boldsymbol{g}}

\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\renewcommand{\dim}{\mrm{dim}}
\newcommand{\Th}{\mathrm{T}_h}
\renewcommand{\div}{\mrm{div}}
\DeclareMathOperator{\T}{T} % Local Transmission operator

\DeclareMathOperator{\V}{\mathcal{V}_{\Gamma}} % weakly singular operator
\DeclareMathOperator{\K}{\mathcal{K}_{\Gamma}} % double layer potential or its adjoint
\DeclareMathOperator{\Kprime}{\tilde{\mathcal{K}}_{\Gamma}} % double layer potential adjoint
\DeclareMathOperator{\W}{\mathcal{W}_{\Gamma}} % hypersingular operator


%% \newcommand{\Bh}{\mathrm{B}_h}
%% \newcommand{\Ah}{\mathrm{A}_h}
%% \newcommand{\Sh}{\mathrm{S}_h}

\newcommand{\Bh}{\mathrm{B}}
\newcommand{\Ah}{\mathrm{A}}
\newcommand{\Sh}{\mathrm{S}}



\newcommand{\Ts}{\mT_{\textsc{s}}}
\newcommand{\Ps}{\mP_{\textsc{s}}}
\newcommand{\Range}{\mrm{Range}}


\newcommand{\calT}{\mathcal{T}}

\newcommand{\dof}{\mathrm{dof}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\supp}{\mathrm{supp}}
\DeclareMathOperator{\diag}{diag} % diagonal


% Name of transmission couplings
% Two domains
\newcommand{\DespresDespres}{\textit{D-D}}
\newcommand{\SchurSchur}{\textit{S-S}}
\newcommand{\SchurYukawa}{\textit{Y-S}}
\newcommand{\YukawaYukawa}{\textit{Y-Y}}
% Three domains
\newcommand{\DespresDespresDespres}{\textit{D-D-D}}
\newcommand{\YukawaSchurDespres}{\textit{Y-S-D}}
\newcommand{\YukawaSchurSchur}{\textit{Y-S-S}}
\newcommand{\YukawaSchurYukawa}{\textit{Y-S-Y}}


% Cite Left and Right Figures
\newcommand{\figpart}[2]{\cref{#1}~(#2)}

\DeclareMathOperator{\DtN}{DtN} % Dirichlet to Neumann operator


\newcommand{\Hdemi}{\mH^{1/2}(\Gamma)} % H^{1/2} space on Gamma (boundary)
\newcommand{\HMdemi}{\mH^{-1/2}(\Gamma)} % H^{-1/2} space on Gamma (boundary)

% \RedeclareMathOperator{\Re}{Re} % real part
% \RedeclareMathOperator{\Im}{Im} % imaginary part  Can not be used because \mrm{Im} already used to denote the image!
\renewcommand{\Re}{\mathfrak{Re}} % real part
\renewcommand{\Im}{\mathfrak{Im}} % imaginary part


%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{defn}{Definition}[section]
\newtheorem{lem}[defn]{Lemma}
\newtheorem{thm}[defn]{Theorem}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{cor}[defn]{Corollary}
\newtheorem{rem}[defn]{Remark}
\newtheorem{example}[defn]{Example}
\newtheorem{asum}{Assumption}
\newtheorem{cond}[asum]{Condition}
\newtheorem{remark}{Remark}

% \orcidID macro from springer
\def\orcidID#1{\unskip$^{[#1]}$}% 
